Inverse moment problem for non-Abelian Coxeter double Bruhat cells

We solve the inverse problem for non-Abelian Coxeter double Bruhat cells in terms of the matrix Weyl functions. This result can be used to establish complete integrability of the non-Abelian version of nonlinear Coxeter-Toda lattices in $GL_n$.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{2}

